Tell me what I need to know: Exploring LLM-based (Personalized) Abstractive Multi-Source Meeting Summarization

Meeting summarization is crucial in digital communication, but existing solutions struggle with salience identification to generate personalized, workable summaries, and context understanding to fully comprehend the meetings' content. Previous attempts to address these issues by considering related supplementary resources (e.g., presentation slides) alongside transcripts are hindered by models' limited context sizes and handling the additional complexities of the multi-source tasks, such as identifying relevant information in additional files and seamlessly aligning it with the meeting content. This work explores multi-source meeting summarization considering supplementary materials through a three-stage large language model approach: identifying transcript passages needing additional context, inferring relevant details from supplementary materials and inserting them into the transcript, and generating a summary from this enriched transcript. Our multi-source approach enhances model understanding, increasing summary relevance by ~9% and producing more content-rich outputs. We introduce a personalization protocol that extracts participant characteristics and tailors summaries accordingly, improving informativeness by ~10%. This work further provides insights on performance-cost trade-offs across four leading model families, including edge-device capable options. Our approach can be extended to similar complex generative tasks benefitting from additional resources and personalization, such as dialogue systems and action planning.

==> text/05_Real_World_Scenario.tex <==
\subsection{Real world application - low budget approach}
% \begin{table}[]
%     \centering
%     \small
%     \begin{tabular}{lcccc}
%     \toprule
%     Setup       & INF   & REL   & FAC   & OVR  \\
%     \midrule
%     G-GPT4    & 4.59 & 4.09 & \hl{3.83} & 4.34 \\
%     G-Phi3    & 4.18 & 3.97 & 4.38 & 4.12 \\
%     G-Gemini  & 4.36 & 4.12 & 4.64 & 4.64 \\
%     G-Llama3  & 3.84 & 3.75 & 4.69 & 4.06 \\
%     \midrule
%     GPT4        & 4.17 & 3.90 & 4.53 & 4.03 \\  % 4.47
%     Phi3        & 4.17 & 3.90 & 4.53 & 4.03 \\
%     Gemini      & 4.17 & 3.90 & 4.53 & 4.03 \\
%     Llama3      & 4.17 & 3.90 & 4.53 & 4.03 \\
%     \bottomrule
%     \end{tabular}
%     \caption{LLM-based Likert scoring of the general multi-source meeting summarization pipeline.}
%     \label{tab:budget_pipeline_results}
% \end{table}


\begin{table}[]
    \centering
    \small
    \begin{tabular}{lcccc}
    \toprule
     & G-GPT4    & G-Phi3& G-Gemini   & G-Llama3  \\
    \midrule
    INF     & 4.59      & 4.18  & 4.36  & 3.84\\
    REL     & 4.09      & 3.97  & 4.12  & 3.75\\
    FAC     & \hl{3.83} & 4.38  & 4.64  & 4.69\\
    OVR     & 4.34      & 4.12  & 4.64  & 4.06\\
    \midrule
    Cost in    & 0.00  & 0.00  & 0.00  & 0.00\\
    Cost out    & 0.00  & 0.00  & 0.00  & 0.00\\
    \midrule
    Time    & 0.00  & 0.00  & 0.00  & 0.00\\
    \bottomrule
    \end{tabular}
    \caption{LLM-based Likert scoring of the general multi-source meeting summarization pipeline.}
    \label{tab:budget_pipeline_results_general}
\end{table}




% \subsection{Real world application - low budget approach}
% \begin{table}[]
%     \centering
%     \small
%     \begin{tabular}{lcccccc}
%     \toprule
%     Setup       & INF-P   & REL-P   & FAC   & OVR-P & Cost & Time \\
%     \midrule
%     P-GPT    & 4.44 & 4.12 & 4.48 & 4.84 & 0.00 & 00\\
%     \colorbox{red}{P-Phi}         & 00.00 & 00.00 & 00.00 & 00.00 & 0.00 & 00\\
%     \hl{P-Gem}      & 4.54 & 4.00 & 4.43 & 4.49 & 0.00 & 00\\
%     \hl{P-Lla}       & 3.85 & 3.82 & 4.35 & 4.00 & 0.00 & 00\\
%     \midrule
%     \colorbox{orange}{GPT} & 4.35 & 3.97 & 4.33 & 4.35 & 0.00 & 00\\
%     Phi        & 4.17 & 3.90 & 4.53 & 4.03 & 0.00 & 00\\
%     Gem      & 4.17 & 3.90 & 4.53 & 4.03 & 0.00 & 00\\
%     Lla      & 4.17 & 3.90 & 4.53 & 4.03 & 0.00 & 00\\
%     \bottomrule
%     \end{tabular}
%     \caption{LLM-based Likert scoring of the general multi-source meeting summarization pipeline.}
%     \label{tab:budget_pipeline_results}
% \end{table}

\begin{table}[]
    \centering
    \small
    \begin{tabular}{lcccc}
    \toprule
            & P-GPT4& P-Phi3& P-Gemini   & P-Llama3  \\
    \midrule
    INF     & 4.44  & 0.00  & 4.54  & 3.85\\
    REL     & 4.12  & 0.00  & 4.00  & 3.82\\
    FAC     & 4.48  & 0.00  & 4.43  & 4.35\\
    OVR     & 4.84  & 0.00  & 4.49  & 4.00\\
    \midrule
    Cost in    & 0.00  & 0.00  & 0.00  & 0.00\\
    Cost out    & 0.00  & 0.00  & 0.00  & 0.00\\
    \midrule
    Time    & 0.00  & 0.00  & 0.00  & 0.00\\
    \bottomrule
    \end{tabular}
    \caption{LLM-based Likert scoring of the general multi-source meeting summarization pipeline.}
    \label{tab:budget_pipeline_results_personal}
\end{table}


So far, we have explored new concepts for multi-source summarization and personalization using GPT4, a model that is well suited for such an exploration task and capable of producing good content even with less-than-good inputs \cite{missing}.
In the following, we investigate whether smaller, more efficient versions of LLMs can serve as the backbone for these concepts, allowing their practical implementation.
We, therefore, evaluate the so far best-performing setups of our pipelines, the 'infer' and 'infer+per' versions, using the Phi-3 mini 3.8b 128k (Phi3, suited for smartphone use cases), Gemini Flash 1.5 (Gemini), and Llama 3 8b (Llama3, strongest academic model) models on one-third of \dataset{} to generate a general summary and a summary for the 'Project Manager' participant.
As Llama3 cannot process the entire transcript at once, we employ a sequential chunking and sub-summary approach following \citet{BOOOOOKSCORE}, updating a global summary with each chunk processed.
All models are accessed via APIs (GPT4, Phi3: Azure; Gemini: Google Cloud; Llama3: Groq).


Quantitative results (\Cref{tab:budget_pipeline_results_general}) show that all backbone models benefit from our multi-source summarization pipeline, with larger models scoring higher.
Gemini's strong performance is expected considering the model's size, while Phi3 surprisingly often outperforms the larger Llama model.
Qualitatively, Gemini produces more high-level, concise summaries, lacking the necessary depth.
Phi3 generates summaries close to GPT4's quality, occasionally lacking detail.
Further, Phi3 sometimes generates fewer than five questions and insertions, limiting the multi-source aspect.
Llama3 struggles with repetition and representing the meeting's structure.

The extracted personalities show significant overlap across models.
Phi3 and GPT4 produce similar-length personas, while Gemini and Llama3 generate longer, more detailed ones.
Analysis of summaries reveals that Phi3 often describes participant actions rather than summarizing a persona's interests.
Llama3 struggles with contextualizing salient content for specific users, including irrelevant information, which aligns with its low INF and REL scores in \Cref{tab:budget_pipeline_results_personal}.
Gemini handles personalization well but tends towards high-level summaries again, omitting important details.

While GPT4 and Gemini perform the best, they are also the most costly models (\$0.5 and \$0.45 per summary).
Llama3 and Phi3 have lower costs (\$0.21 and \$0.18 per summary) primarily due to their smaller model sizes, and can also be run locally.
Especially Phi3 is designed to be run on even weaker hardware, potentially reducing costs and allowing for offline usage.

The different model sizes also become notable in the inference speed, as GPT4 takes roughly XX seconds per call, accumulating to $\sim$ 85 seconds for personalized summaries.
This contrasts with the cheapest model, Phi3, which takes an average of 20 seconds for a personalized summary.
Gemini is in the upper third of this range with $\sim$45 seconds.
Llama3 takes notable time, close to Gemini, with $\sim$43 seconds, likely due to the additional model calls required to process all inputs larger than the context size of 8000 tokens.

% Cost analysis reveals OpenAI, Google, and Microsoft models have comparable API pricing, while Phi-3 and Llama 3 can run on a single GPU, potentially reducing costs.
% GPT4 has the slowest inference speed at 85 seconds per summary, contrasting with Phi3's rapid 20 seconds per summary.
% Open-source models like Phi3 and Llama3 offer additional advantages through optimization techniques such as quantization, pruning, and distillation, providing greater control over memory usage and inference speed. 

Considering performance, cost, and time, we conclude that GPT4 offers the best performance for unrestricted scenarios, while Phi3 is ideal for highly computational and time-constrained environments. It allows for good-quality on-device and offline multi-source summaries.
However, Phi3 requires additional quality assurance systems like feedback loops \cite{EMNLP}, especially for personalization.
Gemini performs close to GPT4 with a slight price advantage.
Llama3, using the current chunking approach, lags in quality and needs further research. 
%In summary, GPT-4 leads in performance, Phi3 provides the most efficient option, and Llama3 offers a promising alternative with room for improvement, allowing flexible implementation based on specific use-case requirements.


% Cost-wise, the models by openai, Google, and Microsoft can be accessed via a dedicated API at similar costs, while Phi-3 and Llama 3 can be also run on a single GPU.
% The inference speed is the slowest for GPT4 with an average of 10 sec per call, 60 secs per summary.
% On the other hand, Phi-3 responds the quickest due to the small size, with an average of 30 seconds per summary.
% Phi-3 and Llama 3 further allow due to their open-source that they can be used with various model optimization techniques such as quantization, pruning, and distilling, allowing to further control the memory usage and inference speed, where as the closed models are fix black boxes.
% Considering these additional metrics, we conclude that a GPT4 base approach is best performing setup, Phi-3 the best budget version, and Llama 3 a good and balanced competitor.


==> text/06_Discussion_and_Impact.tex <==
Our summarization pipeline employs a modular architecture that enables enhanced scalability regarding input documents to consider and adaptability to diverse use cases, such as single-source summarization, multi-source summarization, and personalization.
The pipeline, especially the CoT prompting, supports interpretability and explicit control over the individual components.
We anticipate that our approach will aid other industrial use cases where text generation benefits from considering additional input sources, such as story generation, planning, or ??

